Multi-View Photometric Stereo: A Robust Solution and Benchmark Dataset for Spatially Varying Isotropic Materials

We present a method to capture both 3D shape and spatially varying reflectance with a multi-view photometric stereo (MVPS) technique that works for general isotropic materials. Our algorithm is suitable for perspective cameras and nearby point light sources. Our data capture setup is simple, which consists of only a digital camera, some LED lights, and an optional automatic turntable. From a single viewpoint, we use a set of photometric stereo images to identify surface points with the same distance to the camera. We collect this information from multiple viewpoints and combine it with structure-from-motion to obtain a precise reconstruction of the complete 3D shape. The spatially varying isotropic bidirectional reflectance distribution function (BRDF) is captured by simultaneously inferring a set of basis BRDFs and their mixing weights at each surface point. In experiments, we demonstrate our algorithm with two different setups: a studio setup for highest precision and a desktop setup for best usability. According to our experiments, under the studio setting, the captured shapes are accurate to 0.5 millimeters and the captured reflectance has a relative root-mean-square error (RMSE) of 9%. We also quantitatively evaluate state-of-the-art MVPS on a newly collected benchmark dataset, which is publicly available for inspiring future research.

==> tex/reflectance.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.45\linewidth]{Figures/angles.pdf}
	\caption{Definition of $\theta_h, \theta_d$ and $\phi$, which an isotropic BRDF is defined over as a 3D lookup table.}\label{fig:parameters}
\end{figure}

\section{Reflectance Capture}\label{sec:BRDF}

We assume the surface reflectance can be represented by a linear combination of several (K=2) basis isotropic BRDFs. Once the 3D shape is reconstructed, we follow \cite{Lawrence2006} to estimate the basis BRDFs and their mixing weights at each point on the surface. We consider the general tri-variant isotropic BRDF, which is a function of $\theta_h, \theta_d, \phi$ as shown in
\figref{parameters}. We discretize $\theta_h, \theta_d$ and $\phi$ into $90, 2$ and $5$ bins respectively all in the interval $[0,\pi/2]$. Please refer to \cite{Romeiro2010} for a justification of
choosing this interval. Hence, a BRDF is represented as a $900 \times 1$ vector by concatenating its values at these bins.


We build an $N\times M$ observation matrix $\ve{V}$, and factorize it into a matrix of mixing weights $\ve{W}$ and a matrix of basis BRDFs $\ve{H}$ as,
\begin{displaymath}
\ve{V}_{N\times M} = \ve{W}_{N\times K} \ve{H}_{K \times M}.
\end{displaymath}
$M=900$ is the dimension of a BRDF. $N$ is the number of 3D points. Each row of $\ve{V}$ represents the observed BRDF of a surface point. In constructing the matrix $\ve{V}$, we avoid pixels observed from slanted viewing directions (the angle between viewing direction
and surface normal is larger than $40$ degrees in our
implementation), where a small shape reconstruction error can  cause a big change in their projected image positions. $\ve{V}$ contains missing elements because of incomplete observation. We apply the Alternating Constrained Least Squares (ACLS) algorithm
\cite{Lawrence2006} to iteratively compute the rows of $\ve{W}$ and columns of $\ve{H}$.


To further improve reflectance capture accuracy, we first compute $\ve{H}$ from a subset of precisely reconstructed 3D points, whose reconstructed normals from different combinations of azimuth angles are consistent within $1.5$ degrees. We then fix $\ve{H}$ and compute $\ve{W}$ at all surface points.


